Do Llamas Work in English? On the Latent Language of Multilingual Transformers

We ask whether multilingual language models trained on unbalanced, English-dominated corpora use English as an internal pivot language -- a question of key importance for understanding how language models function and the origins of linguistic bias. Focusing on the Llama-2 family of transformer models, our study uses carefully constructed non-English prompts with a unique correct single-token continuation. From layer to layer, transformers gradually map an input embedding of the final prompt token to an output embedding from which next-token probabilities are computed. Tracking intermediate embeddings through their high-dimensional space reveals three distinct phases, whereby intermediate embeddings (1) start far away from output token embeddings; (2) already allow for decoding a semantically correct next token in the middle layers, but give higher probability to its version in English than in the input language; (3) finally move into an input-language-specific region of the embedding space. We cast these results into a conceptual model where the three phases operate in "input space", "concept space", and "output space", respectively. Crucially, our evidence suggests that the abstract "concept space" lies closer to English than to other languages, which may have important consequences regarding the biases held by multilingual language models.

==> BoolQ.tex <==
\xhdr{BoolQ} Another way to make languages distinguishable from each other is to consider the narrow, well-delimited scenario of binary question answering. The syntax of such questions makes it possible to design a prompt for which a one-token completion suffices to determine whether the answer is ``yes'' or ``no'' (or its equivalent in the language of the question).
As a source for binary questions we leverage the BoolQ dataset~\cite{clark2019boolq}. In BoolQ each question is accompanied with a passage providing the necessary information required to answer the question. 
%From the 16,000 binary questions contained in BoolQ, 
We sample 200 questions and passages from BoolQ, and translate them into French, German, and Russian using DeepL\footnote{https://www.deepl.com/translator}. %We have chosen these languages because they are among the most frequent languages in \llama's training data, they use words for ``yes'' and ``no'' that are mutually distinct across languages, and each of these languages is spoken by at least one author of this paper, which facilitated the inspection of results during development. 

To distinguish the languages, we construct sets $T_{\ell}$ of binary-answer tokens. We start by translating yes/no into $\ell$ (German: ja/nein, French: oui/non, Russian: да/нет). Since, words may be represented as sequences of multiple tokens, we also consider all single-token prefixes of the yes/no words. E.g., ``nein'' may be tokenized as ``ne-in'', so we count the first token ``ne'' as indicating German. 

Furthermore, we include all capitalization variants and tokens with and without leading whitespace (e.g., Yes, \_Yes). Importantly, we discard incomplete prefixes (i.e., prefixes that are not themselves complete equivalents of yes or no) that are shared across languages, such that no unique language could be inferred from the prefix (e.g., ``n'' is not included, as it could be the start of ``no'' (EN), ``nein'' (DE), or ``non'' (FR)). 
Searching \llama{}'s vocabulary according to these criteria results in Appendix~\ref{app:info}~Tab.~\ref{tab:boolq-yes-no-tokens}, where we provide a complete list of the binary-answer tokens used. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For BoolQ, we have a better approximation of the language probability by considering all binary-answer tokens in the respective languages $T_{\ell}$. As a result we have
\begin{eqnarray}
P(\text{lang}=\ell) &=& \sum_{t \in T_{\ell}} P(\text{next}=t),
\end{eqnarray}
for each lang $\ell$ and layer $j$ by summing up the tokens corresponding to ``yes'' or ``no'' in lang $\ell$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\xhdr{BoolQ answer accuracy} For BoolQ, we also compute the accuracy for each decoded answer, for each input language $\ell$ and layer $j$. To decode an answer from an intermediate layer, we split $T_{\ell}$ into yes tokens $Y_{\ell}$ and no tokens $Y_{\ell}$ and compute 
\begin{equation}
r = \argmax_{t \in T_{\ell}} P(\text{next}=t)
\end{equation}
and interpret $r$ as yes if $r \in Y_{\ell}$ and as no if $r \in N_{\ell}$. Then, the accuracy is defined as the fraction of correct responses $r$ as usual.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{BoolQ}
The final task is binary question answering. Unlike the previous tasks, the output vocabulary is restricted to two tokens ``yes'' and ``no''. Consequently, the probability of the language is limited to these two tokens in the respective languages (in the Appendix \ref{app:info} Tab.~\ref{tab:boolq-yes-no-tokens} we include the tokens used). 
Across all languages and model sizes the intermediate beliefs about the answer are first concentrated on English (middle layers) before they change to the language specific counterparts (last layers). Additionally, most of the probability mass falls into the small selected subset of binary-answer tokens, which is indicated by the fact that both $P(\text{lang}=\text{EN})$ as well as $P(\text{lang}=\text{DE})$ almost reach a value of $1$. 
Interestingly, as in the prior examples, in the very last layer the probabilities fall off. Manual inspection of a few examples shows that binary-answer tokens still constitute 
most of the top 10 tokens, however with decreased probability magnitude, which may reflect proper calibration of the last layer for which the language modelling 
head was intended. This is consistent with the entropy pattern displayed in the heatmaps.

\xhdrNoPeriod{Pivot language English?} But, does the fact that the intermediate beliefs concentrate on the English binary-answer tokens imply that English is used as a pivot language? In order to answer this question, we have to consider the accuracy of the decoded answers across layers in the BoolQ task. We define an answer as correct if the argmax over the ``yes'' and ``no'' probabilities is correct. This is shown in Fig.~\ref{fig:boolq_acc}, which depicts the accuracy for English and German across all layers and model sizes. If English was used as a pivot language, we would expect the accuracy to increase in the intermediate layers and then stay fixed. The intuition behind this is that once the English answer is obtained, all that is left to do is to translate it to the input language. However, in contrast to the two previous tasks (translation task and cloze task) where this is the case, this is not what we observe here.

Instead, the accuracy is pretty much exactly 62\% in the intermediate layers, which is the accuracy of always answering ``yes'', and only increases at the very end. Since, we have also observed the same pattern (i.e., English answer being ``yes'' in the intermediate layers) for easier binary question answering tasks, we believe that the pivot-language effect occurs on a coarser scale of granularity than is required for binary question answering, where the correct response is determined by a single bit of information. We also cannot exclude the possibility that this lack of resolution also may be attributed to using the logit lens as intermediate decoding method.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/boolq/7B_de_acc.pdf}
        \caption*{7B}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/boolq/13B_de_acc.pdf}
        \caption*{13B}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/boolq/70B_de_acc.pdf}
        \caption*{70B}
    \end{subfigure}
    \caption{BoolQ accuracy German. There is one column per model size 7B, 13B, and 70B. In each subplot, the x-axis shows the layer index, the y-axis the accuracy. We report the mean over 200 samples from our multilingual BoolQ dataset.}
    \label{fig:boolq_acc}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> junkyard.tex <==
\section{Logit lens plots}
\label{app:info}

Here we provide some additional heatmaps plotted with the tuned lens library~\cite{belrose2023eliciting}.
We provide a complete translation example (including few shot demonstrations) in  Fig.~\ref{fig:translation-llama2-7b-ex-double} and its most relevant part (the last pair) in Fig.~\ref{fig:translation-llama2-7b-ex-double-relevant}.
Similarly, we provide a complete cloze example (including few shot demonstrations) in Fig.~\ref{fig:cloze-llama2-7b-ex-double} and its most relevant part in Fig.~\ref{fig:cloze-llama2-7b-ex-double-relevant}.

 \begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/translation/translation_example_five.png}
    \caption{Intermediate decodings running logit lens on \llama{}-7B when processing a translation example. The y-axis shows the layer index, the x-axis the input tokens, and the color indicates the entropy of the next-token distribution with dark blue representing low- and dark red high entropy.}
    \label{fig:translation-llama2-7b-ex-double}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/translation/translation_example_one.png}
    \caption{Intermediate decodings of last few tokens of running logit lens on \llama{}-7B when processing a translation example (only the relevant part after the demonstrations). The y-axis shows the layer index, the x-axis the input tokens, and the color indicates the entropy of the next-token distribution with dark blue representing low- and dark red high entropy.}
    \label{fig:translation-llama2-7b-ex-double-relevant}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/cloze/cloze_example_full.png}
    \caption{Intermediate decodings running logit lens on \llama{}-7B when processing a cloze example. The y-axis shows the layer index, the x-axis the input tokens, and the color indicates the entropy of the next-token distribution with dark blue representing low- and dark red high entropy.}
    \label{fig:cloze-llama2-7b-ex-double}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/cloze/cloze_example.png}
    \caption{Intermediate decodings of last few tokens of running logit lens on \llama{}-7B when processing an example from the cloze task (only the relevant part after the demonstrations). The y-axis shows the layer index, the x-axis the input tokens, and the color indicates the entropy of the next-token distribution with dark blue representing low- and dark red high entropy.}
    \label{fig:cloze-llama2-7b-ex-double-relevant}
\end{figure*}

\section{Prompt format}
\label{app:prompts}

We provide a short overview of our prompting templates used to perform the experimental evaluation.


%\begin{minted}[mathescape, linenos, numbersep=5pt, gobble=2, frame=lines, framesep=2mm]{text}
%Français: "poupée" - Deutsch: "Puppe" - Русский: "кукла"
%\end{minted}


\lstset{
  literate=%
    {ä}{{\"a}}1
    {ö}{{\"o}}1
    {ü}{{\"u}}1
    {Ä}{{\"A}}1
    {Ö}{{\"O}}1
    {Ü}{{\"U}}1
    {ß}{{\ss}}1
    {ç}{{\c{c}}}1
    {é}{{\'e}}1
    {è}{{\`e}}1
    {à}{{\`a}}1
}

\xhdr{Translation} For the translation task we use 4-shot prompts of the form:

% \begin{minipage}{\textwidth}
\begin{minted}[mathescape, linenos, numbersep=5pt, gobble=0, frame=lines, framesep=2mm, fontsize=\scriptsize, breaklines]{text}
Français: "bouton" - Deutsch: "Knopf"
Français: "poupée" - Deutsch: "Puppe"
Français: "violon" - Deutsch: "Geige"
Français: "tambour" - Deutsch: "Trommel"
Français: "fleur" - Deutsch: "
\end{minted}
% \end{minipage}

Note that all pairs are randomly sampled.

\xhdr{Cloze} For the cloze task we use 2-shot prompts of the form:
% \begin{minipage}{\textwidth}
\begin{minted}[mathescape, linenos, numbersep=5pt, gobble=0, frame=lines, framesep=2mm, fontsize=\scriptsize, breaklines]{text}
"___" ist ein festes Material, das einen Teil der Erdoberfläche bildet. Antwort: "Gestein".
"___" ist ein Gerät, das häufig in Haushalten verwendet wird, um ausgestrahlte Programme und Filme anzusehen. Antwort: "Fernsehen".
"___" ist der Stern im Zentrum des Sonnensystems, der die Erde mit Licht und Wärme versorgt." Antwort: "
\end{minted}
% \end{minipage}

Note that both the demonstrations are randomly sampled.


\xhdr{BoolQ} For BoolQ we use prompts of the form:
% \begin{minipage}{\textwidth}
% \begin{minted}[mathescape, linenos, numbersep=5pt, gobble=0, frame=lines, framesep=2mm, %fontsize=\scriptsize, breaklines]{text}
% Write a response that appropriately completes the request.

% ### Instructions:
% Read the input passage and answer the question: Is elder scrolls online the same as skyrim? Your answer should be "Yes" or "No".

% ### Input:
% As with other games in The Elder Scrolls series, the game is set on the continent of Tamriel. The events of the game occur a millennium before those of The Elder Scrolls V: Skyrim and around 800 years before The Elder Scrolls III: Morrowind and The Elder Scrolls IV: Oblivion. It has a broadly similar structure to Skyrim, with two separate conflicts progressing at the same time, one with the fate of the world in the balance, and one where the prize is supreme power on Tamriel. In The Elder Scrolls Online, the first struggle is against the Daedric Prince Molag Bal, who is attempting to meld the plane of Mundus with his realm of Coldharbour, and the second is to capture the vacant imperial throne, contested by three alliances of the mortal races. The player character has been sacrificed to Molag Bal, and Molag Bal has stolen their soul, the recovery of which is the primary game objective.

% ### Response:
% The answer is "
% \end{minted}
%\end{minipage}


% \begin{minipage}{\textwidth}
\begin{minted}[mathescape, linenos, numbersep=5pt, gobble=0, frame=lines, framesep=2mm, fontsize=\scriptsize, breaklines]{text}
 Schreiben Sie eine Antwort, die die
 Anfrage.
 ### Anweisungen :
 Lesen Sie den Eingangstext und beantworten Sie die Frage: Ist
 elder scrolls online dasselbe wie skyrim? Ihre
 Antwort sollte "Ja" oder "Nein" lauten.
 ### Eingabe :
 Wie bei anderen Spielen der The Elder Scrolls-Reihe ,
 ist das Spiel auf dem Kontinent Tamriel angesiedelt.
 Die Ereignisse des Spiels spielen ein Jahrtausend
 vor denen von The Elder Scrolls V: Skyrim
 und etwa 800 Jahre vor The Elder Scrolls
 I I I : Morrowind und The Elder Scrolls IV:
 Oblivion . Es hat eine weitgehend ähnliche Struktur
 Skyrim, mit zwei separaten Konflikten
 Konflikte, von denen einer das Schicksal der
 das Schicksal der Welt auf dem Spiel steht, und einem
 in dem es um die oberste Macht auf Tamriel geht.
 In The Elder Scrolls Online geht es im ersten
 Kampf gegen den daedrischen Prinzen Molag
 Bal , der versucht, die Ebene von
 Mundus mit seinem Reich Coldharbour zu verschmelzen, und der
 zweiten Kampf geht es um den vakanten kaiserlichen
 Thron zu erobern, um den sich drei Allianzen der
 sterblichen Rassen. Der Spielercharakter wurde
 Molag Bal geopfert, und Molag Bal hat
 seine Seele gestohlen, deren Wiedererlangung das
 das primäre Spielziel ist.
 ### Antwort :
 Die Antwort lautet "
\end{minted}
% \end{minipage}

%\newpage
%\begin{minipage}{\textwidth}
%\begin{minted}[mathescape, linenos, numbersep=5pt, gobble=0, frame=lines, framesep=2mm, fontsize=\scriptsize, breaklines]{text}
% Rédiger une réponse qui complète de manière appropriée la
% demande .
% ### Instructions :
% Lisez le passage d'entrée et répondez à la question : Est-ce que
% elder scrolls online est-il identique à skyrim ? Votre réponse doit être "Oui" ou "Non".
% réponse doit être "Oui" ou "Non" .
% ### Entrée :
% Comme les autres jeux de la série The Elder Scrolls ,
% le jeu se déroule sur le continent de Tamriel.
% Les événements du jeu se déroulent un millénaire
% avant ceux de The Elder Scrolls V : Skyrim
% et environ 800 ans avant The Elder Scrolls
% I I I : Morrowind et The Elder Scrolls IV :
% Oblivion . Sa structure est largement similaire à celle de
% de Skyrim, avec deux conflits distincts se déroulant
% conflits distincts se déroulant en même temps, dont l'un
% le destin du monde en jeu, et l'autre où le
% où l'enjeu est le pouvoir suprême sur Tamriel.
% Dans The Elder Scrolls Online, le premier conflit est contre le Prince Daedrique.
% est contre le prince daedrique Molag
% Bal, qui tente de fusionner le plan de Mundus avec son royaume de
% Mundus avec son royaume de Coldharbour, et la deuxième
% deuxième est de s'emparer du trône impérial vacant
% impérial vacant, contesté par trois alliances de
% races mortelles . Le personnage du joueur a été
% sacrifié à Molag Bal, et Molag Bal lui a volé son âme.
% a volé son âme, dont la récupération est l'objectif
% l'objectif principal du jeu .
% ### Réponse :
% La réponse est "
%\end{minted}
%\end{minipage}

%\begin{minipage}{\textwidth}
%\begin{minted}[mathescape, linenos, numbersep=5pt, gobble=0, frame=lines, framesep=2mm, fontsize=\scriptsize, breaklines]{text}
% Напишите ответ, который надлежащим образом завершает
% запрос .
% ### Инструкции :
% Прочитайте вводный отрывок и ответьте на вопрос: Является ли
% elder scrolls online то же самое, что и skyrim? Ваш
% ответ должен быть "Да" или "Нет" .
% ### Вводные данные :
% Как и другие игры серии The Elder Scrolls ,
% действие игры разворачивается на континенте Тамриэль.
% События игры происходят за тысячелетие
% до событий The Elder Scrolls V: Skyrim
% и примерно за 800 лет до событий The Elder Scrolls
% I I I : Morrowind и The Elder Scrolls IV:
% Oblivion . По своей структуре она в целом похожа
% на Skyrim, с двумя отдельными конфликтами
% протекающих одновременно, один из которых
% судьба мира на волоске, и один
% где наградой является верховная власть в Тамриэле.
% В The Elder Scrolls Online основная борьба
% борьба с даэдрическим принцем Молагом
% Баль, который пытается объединить плоскость
% Мундус со своим королевством Колдхарбор, и
% вторая - за вакантный императорский
% трон, за который борются три союза
% смертных рас. Персонаж игрока был
% принесен в жертву Молагу Балу, а Молаг Бал
% украл его душу, возвращение которой является
% главная цель игры.
% ### Ответ :
% Ответ: "
%\end{minted}
%\end{minipage}


Table~\ref{tab:boolq-yes-no-tokens} contains the exact list of yes/no tokens used to calculate language probabilities and accuracies for the BoolQ task.

 \begin{table}
     \centering
     \begin{tabular}{ll}
         \toprule
         English & Yes, YES, yes, \_Yes, \_YES, \_yes \\
          ~~(en)&  No, NO, no, \_No, \_NO, \_no\\
         \midrule 
         German & ja, J, j, \_Ja, \_ja, \_J, \_j   \\
          ~~(de)& Ne, NE, ne, \_nei, \_Ne, \_NE, \_ne  \\
         \midrule 
         French & OU, ou, O, o, \_ou, \_O, \_o \\
          ~~(fr)&  Non, non, \_Non, \_non\\
         \midrule 
         Russian & да, Д, д, \_Да, \_да, \_Д, \_д \\
          ~~(ru) &  нет, Не, не, Н, н, \_Не, \_не, \_Н, \_н\\
         \bottomrule
     \end{tabular}
     \caption{Tokens that we consider as the binary-answer tokens in the respective language. We denote leading whitespaces by \_.}
     \label{tab:boolq-yes-no-tokens}
 \end{table}

For BoolQ, we also include the accuracy plots in Fig.~\ref{fig:boolq_acc_all} and in addition the accuracy numbers for BoolQ after the final layer in Tab.~\ref{tab:accuracy}. As can be seen, on our sample we achieve accuracy comparable to the one reported in \cite[Tab.~18]{touvron2023llama} for a \llama{}-30B variant.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/lens_double_columns.png}
    \caption{Intermediate decodings of last few tokens of running logit lens on \llama{}-7B when processing an example from the BoolQ task (only the relevant part). The y-axis shows the layer index, the x-axis the input tokens, and the color indicates the entropy of the next-token distribution with dark blue representing low- and dark red high entropy.}
    \label{fig:boolq-llama2-7b-ex-double}
\end{figure*}


\begin{figure*}[ht!]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/7b_de_fr_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (DE->FR)}
         \includegraphics[width=\textwidth]{figures/translation/13b_de_fr_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.343\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/70b_de_fr_probas_ent.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/7b_de_ru_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (DE->RU)}
         \includegraphics[width=\textwidth]{figures/translation/13b_de_ru_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.343\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/70b_de_ru_probas_ent.pdf}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/7b_fr_de_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (FR->DE)}
         \includegraphics[width=\textwidth]{figures/translation/13b_fr_de_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.343\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/70b_fr_de_probas_ent.pdf}
     \end{subfigure}

    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/7b_fr_ru_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (FR->RU)}
         \includegraphics[width=\textwidth]{figures/translation/13b_fr_ru_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.343\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/70b_fr_ru_probas_ent.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/7b_ru_de_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (RU->DE)}
         \includegraphics[width=\textwidth]{figures/translation/13b_ru_de_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.343\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/70b_ru_de_probas_ent.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/7b_ru_fr_probas_ent.pdf}
         \caption*{7B}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (RU->FR)}
         \includegraphics[width=\textwidth]{figures/translation/13b_ru_fr_probas_ent.pdf}
         \caption*{13B}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.343\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/70b_ru_fr_probas_ent.pdf}
         \caption*{70B}
     \end{subfigure}


     \caption{Figures illustrate the translation task where \llama{} 7B, 13B, and 70B are tasked with translating a word from non-English input language to output language. There is one column per model size. The x-axis shows the layer number of the model, and the y-axis the total probability mass falling on the correct token across languages. The yellow line illustrates the probability of the correct target word in English and the blue line shows it for the non-English output language. We do not include the probability the input language since it is zero throughout. Means and 95\% Gaussian confidence intervals have been computed over the 70 examples.}
     \label{fig:translation}
 \end{figure*}


\begin{figure*}[ht!]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/same/7b_de_de_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (DE->DE)}
         \includegraphics[width=\textwidth]{figures/same/13b_de_de_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/same/70b_de_de_attn_mlp_delta.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/same/7b_fr_fr_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (FR->FR)}
         \includegraphics[width=\textwidth]{figures/same/13b_fr_fr_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/same/70b_fr_fr_attn_mlp_delta.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/same/7b_ru_ru_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (RU->RU)}
         \includegraphics[width=\textwidth]{figures/same/13b_ru_ru_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/same/70b_ru_ru_attn_mlp_delta.pdf}
     \end{subfigure}


     \caption{Figures illustrate the copying task where \llama{} 7B, 13B, and 70B are tasked with copying a non-English word. We analyse the contributions of attention layers and MLP layers separately. There is one column per model size. The x-axis shows the layer number of the model, and the y-axis the total probability mass difference on the correct token across languages. The yellow line illustrates the probability of the correct target word in English and the blue line shows it for the non-English output language. Means and 95\% Gaussian confidence intervals have been computed over the 70 examples.}
     \label{fig:copy_diff}
 \end{figure*}

  \begin{figure*}[ht!]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/7b_de_fr_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (DE->FR)}
         \includegraphics[width=\textwidth]{figures/translation/13b_de_fr_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/70b_de_fr_attn_mlp_delta.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/7b_de_ru_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (DE->RU)}
         \includegraphics[width=\textwidth]{figures/translation/13b_de_ru_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/70b_de_ru_attn_mlp_delta.pdf}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/7b_fr_de_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (FR->DE)}
         \includegraphics[width=\textwidth]{figures/translation/13b_fr_de_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/70b_fr_de_attn_mlp_delta.pdf}
     \end{subfigure}

    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/7b_fr_ru_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (FR->RU)}
         \includegraphics[width=\textwidth]{figures/translation/13b_fr_ru_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/70b_fr_ru_attn_mlp_delta.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/7b_ru_de_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (RU->DE)}
         \includegraphics[width=\textwidth]{figures/translation/13b_ru_de_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/70b_ru_de_attn_mlp_delta.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/7b_ru_fr_attn_mlp_delta.pdf}
         \caption*{7B}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Translation (RU->FR)}
         \includegraphics[width=\textwidth]{figures/translation/13b_ru_fr_attn_mlp_delta.pdf}
         \caption*{13B}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/translation/70b_ru_fr_attn_mlp_delta.pdf}
         \caption*{70B}
     \end{subfigure}


     \caption{Figures illustrate the translation task where \llama{} 7B, 13B, and 70B are tasked with translating a word from non-English input language to output language. We analyse the contributions of attention layers and MLP layers separately. There is one column per model size. The x-axis shows the layer number of the model, and the y-axis the total probability mass difference on the correct token across languages. The yellow line illustrates the probability of the correct target word in English and the blue line shows it for the non-English output language. We do not include the probability the input language since it is zero throughout. Means and 95\% Gaussian confidence intervals have been computed over the 70 examples.}
     \label{fig:translation_diff}
 \end{figure*}

 \begin{figure*}[ht!]
     \centering
     
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cloze/7b_de_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Cloze task (DE)}
         \includegraphics[width=\textwidth]{figures/cloze/13b_de_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cloze/70b_de_attn_mlp_delta.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cloze/7b_fr_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Cloze task (FR)}
         \includegraphics[width=\textwidth]{figures/cloze/13b_fr_attn_mlp_delta.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cloze/70b_fr_attn_mlp_delta.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cloze/7b_ru_attn_mlp_delta.pdf}
         \caption*{7B}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \caption{Cloze task (RU)}
         \includegraphics[width=\textwidth]{figures/cloze/13b_ru_attn_mlp_delta.pdf}
         \caption*{13B}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cloze/70b_ru_attn_mlp_delta.pdf}
         \caption*{70B}
     \end{subfigure}
     \caption{Figures show the same plots only for the cloze task where the correct token is defined in a fill-in-the-blank setting.  We analyse the contributions of attention layers and MLP layers separately. There is one column per model size. The x-axis shows the layer number of the model, and the y-axis the total probability mass difference on the correct token across languages. In the plots, we illustrate the results for German. Means and 95\% Gaussian confidence intervals have been computed over the 70 examples.}
     \label{fig:cloze_diff}
 \end{figure*}

 
 \begin{figure*}[ht!]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/boolq/7B_de_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
        \caption{BoolQ (DE)}
         \includegraphics[width=\textwidth]{figures/boolq/13B_de_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.343\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/boolq/70B_de_probas_ent.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/boolq/7B_en_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
        \caption{BoolQ (EN)}
         \includegraphics[width=\textwidth]{figures/boolq/13B_en_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.343\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/boolq/70B_en_probas_ent.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/boolq/7B_fr_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
        \caption{BoolQ (FR)}
         \includegraphics[width=\textwidth]{figures/boolq/13B_fr_probas_ent.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.343\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/boolq/70B_fr_probas_ent.pdf}
     \end{subfigure}

     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/boolq/7B_ru_probas_ent.pdf}
         \caption*{7B}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
        \caption{BoolQ (RU)}
         \includegraphics[width=\textwidth]{figures/boolq/13B_ru_probas_ent.pdf}
         \caption*{13B}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.343\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/boolq/70B_ru_probas_ent.pdf}
        \caption*{70B}
     \end{subfigure}

  
     \caption{Figures show BoolQ results for English, German, French, Russian inputs. Means and 95\% Gaussian confidence intervals have been computed over a sample of 200 questions.}
     \label{fig:boolq}
 \end{figure*}

\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/boolq/7B_de_acc.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \caption{BoolQ (DE)}
        \includegraphics[width=\textwidth]{figures/boolq/13B_de_acc.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/boolq/70B_de_acc.pdf}
    \end{subfigure}

    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/boolq/7B_fr_acc.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \caption{BoolQ (FR)}
        \includegraphics[width=\textwidth]{figures/boolq/13B_fr_acc.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/boolq/70B_fr_acc.pdf}
    \end{subfigure}

    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/boolq/7B_ru_acc.pdf}
        \caption*{7B}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \caption{BoolQ (RU)}
        \includegraphics[width=\textwidth]{figures/boolq/13B_ru_acc.pdf}
        \caption*{13B}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/boolq/70B_ru_acc.pdf}
        \caption*{70B}
    \end{subfigure}
    \caption{BoolQ accuracy German, French, Russian. There is one column per model size 7B, 13B, and 70B. In each subplot, the x-axis shows the layer index, the y-axis the accuracy. We report the mean over 200 samples from our multilingual BoolQ dataset.}
    \label{fig:boolq_acc_all}
\end{figure*}

\begin{table}[h]
    \centering
    \begin{tabular}{lrrrr}
    \toprule
    %Baselines &  &  \\ \hline
    %yes & 0.62 & \\
    %no & 0.38 & \\
    %\llama{} 30 B & 0.71 & \\
        & en   & de   & fr   & ru   \\\hline
    Llama-7B  & 0.64 & 0.64 & 0.63 & 0.62 \\ 
    Llama-13B & 0.68 & 0.73 & 0.66 & 0.62 \\
    Llama-70B & 0.75 & 0.76 & 0.73 & 0.62 \\\bottomrule 
    \end{tabular}
    \caption{Accuracy after the final layer with English, German, French, Russian inputs. Baselines: Always yes achieves 0.62 and a \llama{}-30B~\cite{touvron2023llama} achieves 0.71 in the original BoolQ. Note that here we only use the binary-answer tokens of the respective language for the accuracy computation.} 
    \label{tab:accuracy}
\end{table}

==> old/OLD_TEXT.tex <==
Our main findings are depicted in the Fig.~\ref{fig:combined_probs_entropy}, which shows the development of the 
language probabilities $P(\text{lang}=\ell)$ and $P(\text{lang}=\lang{EN})$ along the layers. 
For the translation task we only consider translations between French and German, and for the repeat word- and cloze tasks we only include German input text. All results are illustrated in \Figref{fig:combined_probs_entropy}. 
% It contains a subplot for English and German for each \llama{} size 7B, 13B, and 70B.
In each subplot, the x-axis shows the layer index, the y-axis the total probability mass falling into either the English or the 
language specific version of the three tasks.
We include results for the other languages (Russian and French) in Appendix~\ref{app:results}. 


\subsection{Repeat word task}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Translation task}
The first task evaluates simple translation. %By providing the model with a 4-shot prompt for the translation task~(see Appendix~\ref{app:prompts} for details), we evaluate the prediction for the fifth translation pair. 
\Figref{fig:combined_probs_entropy} (a) illustrates the probability of the logit lens decoding the correct translation in English and German across the layers of the models. 
%Since the logit lens employs the language modelling head from the last layer without retraining to the intermediate layers, the decoded probabilities are at best an approximation of the true beliefs of the model after each layer, the further away from the last layer the more so. Therefore, the first few layers (the left side of each subplot) probably can safely be ignored. This is also supported by Fig.~\ref{fig:combined_entropy}, which shows that the entropy of the next-token distribution is very high in the early layers and only decreases in the middle ones.
For 7B the intermediate decodings begin to assign probability mass the correct translation in English at layer 16. 
This probability mass on the English translation remains until layer 27 when the logit lens begins to decode to the target language of German. This pattern -- noise in the early layers, English in the middle, German in the end -- continues for the 13B model (English between 16 to 36, and German after layer 36) and for the 70B model (English between 40 to 72, and German after layer 72). 
% We denote this layer where the languages change as the transition layer. 

In addition to the probability density, the entropy is included as a heatmap above the plot. We observe the same pattern for all sizes, high entropy in the early layers, which drops significantly in the middle when the probability mass is on the English token, then when the probabilities change from English to German there is a small increase in entropy that then slowly drops again until the last layer. For 7B, the entropy is 12 until layer 15, then drops all the way to about 1, until it starts slightly increasing again from layer 23 to 26 to a value of about 3 and finally drops again to less than 2.

\subsection{Cloze task}
In the cloze task, the model is required to predict a object noun token based on its description~(see Appendix~\ref{app:prompts} for details). Similar to translation, row (b) in \Figref{fig:combined_probs_entropy} shows the probability of the correct token being decoded in German and English. We observe the same pattern as in the translation task, where following layer 15 (13B: 16, 70B: 39), the logit lens begins to decode the correct masked token in English, and then following layer 26 (13B: 33, 70B: 62), it predicts the correct token in German. In this task, the probability of the correct token is around 10\% lower than in the translation task, which is due to the more ambiguous nature of the cloze task. The entropy also follows the same pattern as in the translation task.

